Blockchain Simulators: A Systematic Mapping Study

Recently, distributed ledger technologies like blockchain have been proliferating and have attracted interest from the academic community, government, and industry. A wide range of blockchain solutions has been introduced, such as Bitcoin, Ethereum, and Hyperledger technologies in the literature. However, tools for evaluating these solutions and their applications are still lacking, limiting the exploration of their potentiality and associated challenges/limitations. That is, experimenting with real blockchain networks usually requires a solid budget; and thus, sophisticated blockchain simulators can facilitate designing and evaluating solutions before the actual implementation stage. The quality of such simulators depends on several factors such as usability, reliability, provided capabilities, and supported features. This paper aims to provide a systemic mapping review of blockchain simulators focusing on these quality factors. This paper also sheds light on the configuration parameters (inputs) and produced metrics (outputs) supported by each simulator. Furthermore, it investigates which metrics supported by each simulator are scientifically validated/evaluated. Moreover, code quality comparison is carried out to assess the source code of the covered simulators. The results reveal that no simulator fully covers the wide operational range of features and capabilities of existing blockchain technologies. However, several promising efforts exist in the domain of blockchain simulation with interesting and useful features. Finally, we discuss the subject of blockchain simulation and provide our insight into the matter.

==> edit.tex <==
\subsubsection{Network layer}
\begin{itemize}
    \item (P1) Total number of nodes configured by the user.
    \item (P1.1) Regions of nodes (unit: geographical) representing the geographical location of each node.
    \item (P2) Total number of connections for each node representing the number of possible connections. Each node may have a different number of connections.
    \item (P3) Average block propagation delay (unit: seconds) representing average time delayed in the propagation process of each block.
    \item (P4) Average transaction propagation delay (unit: seconds) representing the average time delayed in the propagation process of each transaction  configured by the user.
    \item (P5) Average bandwidth among regions in the network (unit: bits per second): This represents the average bandwidth assumed for the simulated network  configured by the user.
    \item (P6) Average latency among the simulated regions (unit: seconds): This represents the average latency assumed for the simulated network  configured by the user.
    \item (P7) Payload transaction size (unit: Megabyte): This represents the maximum transaction size configured by the user.
    \item (P8) Block size (unit: Megabyte): This represents the maximum block size configured by the user. Note that not all block sizes may reach this limit.
    \item (M1) Average block size: This represents the average block sizes simulated in the chain simulated in the simulator.
    \item (M2) Average block propagation time: This represents the average time taken by the simulator to propagate blocks, simulated in the simulator, in the chain.
    \item (M3) Average transaction propagation time: This represents the average time taken by the simulator to propagate transaction in the simulated chain.
    \item (M4) Throughput (unit: Tx/second): This represents the throughput taken by the simulator to the end of the simulations.
\end{itemize}
\subsubsection{Data layer}
    \begin{itemize}
    \item (P9) Generate random transactions (unit: Integer of Tx per second): This represents the ability to generate automatically generated transactions.
    \item (M5) Chain of block: This represents the resulting chain from the simulator at the end of the simulation.
    \item (M6) Security: This represents the security assessed by the simulator at the end of the simulation.
    \end{itemize}
\subsubsection{Consensus layer}
    \begin{itemize}
    \item (P10) A Average mining power (Hash Rate): This represents the average mining power configured by the user.
    \item (P11) PoW consensus Algorithm: This represents the ability of the simulator to implement PoW consensus algorithm. 
    \item (P12) Other consensus Algorithm: This represents the ability of the simulator to implement other consensus algorithms than PoW.
    \item (P13) Average transaction fee (unit: cryptocurrency): This represents the average transaction fees configured by the user.
    \item (P14) Average time for creating a block; aka Block Interval (unit: seconds): This represents the average time configured by the user needed to create a block.
    \item (M7) Average block interval: This represents the average time taken, for the blocks to accept transactions, by simulator at the end of the simulation.
    \item (M8) Number of generated blocks:  This represents the total number of generated blocks in the simulator  at the end of the simulation.
    \item (M9) Number of mined blocks: This represents the total number of mined blocks by the simulator at the end of the simulation.
    \item (M10) Rate of orphan blocks (unit: percentage): This represents the percentage of the orphan blocks by the simulator at the end of the simulation.
    \item (M11) Fork Resolution: This represents whether the simulator maintain the history of blockchain to determine forks occurred as protocol change.
    \end{itemize}
\subsubsection{Incentive layer}
    \begin{itemize}
    \item (P15) Reward for mine a new block (unit: cryptocurrency): This represents the amount of reward configured by the user to mine a block.
    \item (M12) Reward for miner (unit: cryptocurrency): This represents the amount of reward consumed by the simulator at the end of the simulation.
    \end{itemize}
\subsubsection{Execution layer}
    \begin{itemize}
    \item (M13) Time of executing a contract (unit: seconds): This represents the time taken by the simulator to execute a contract.
    \item (M14) Validation of contract and execution time: This represents how the simulator validates the contract.
    \end{itemize}
\subsubsection{Application layer}
\begin{itemize}
    \item (P16) Simulation run time (unit: seconds): This represents the configured simulation time by the user.
    \item (M15) Resources usage: This represents how the simulator keep track of the resource usage and utilization.
    \item (M16) Simulation time (unit: seconds): This represents the actual  time taken by the simulator to the end of the simulation.
    \end{itemize}
    
    \begin{table}[h]
		\renewcommand{\arraystretch}{0.8}
		\centering
		\caption{Searching and screening results.}
		\label{fig:steps}
		\footnotesize{
		\begin{tabular}{ p{0.15\textwidth} p{0.3\textwidth} }
			\hline
		    Searching phase & The number of all found paper is ()  \\
			\hline
			Screening phase & The number of papers selected based on their titles and/or abstract is ()  \\
			                & The number of papers after removing duplication is ()  \\
			                & The number of papers selected after reading the whole paper is ()  \\
			\hline
		    Final phase & The final number of papers included in the study is ()  \\
			\hline
		
		\end{tabular}
		}
	\end{table}
	
	
	\begin{table}[h]
		\renewcommand{\arraystretch}{0.8}
		\centering
		\caption{Search queries.}
		\label{Search queries.}
		\footnotesize{
		\begin{tabular}{ p{0.15\textwidth} p{0.3\textwidth} }
			\hline
		Scientific Database & Query Strings  \\
			\hline
			ACM Digital library & [Title: blockchain] AND [Title: simulator] OR [Abstract: blockchain] AND [Abstract: simulator]\\
			\hline
		    IEEE Xplore & ("Document Title":'Blockchain' AND "Document Title":'Simulator') OR ("Abstract":'Blockchain' AND "Abstract":'Simulator') \\
			\hline
			Springer & "blockchain"  AND  "simulator"  \\
			\hline
			Scopus &  TITLE ( blockchain  AND  simulator ) OR ABS ( blockchain  AND  simulator )\\
			\hline
		\end{tabular}
		}
	\end{table}




==> test.tex <==
\begin{figure*}[h]
	\centering
\includegraphics[scale=0.42]{fig/Parameters and metrics diagram.png}
	\caption{The set of parameters and metrics associated with each layer. The middle part represents blockchain layers and their interconnections. The left part represents the set of parameters invoked in each layer while the right part represents the set of metrics invoked in each layer.}
	\label{ParMetLayers}
\end{figure*}

\begin{figure*}[th]
\centering
\begin{tikzpicture}[ ->,>=stealth', shorten >=1pt, auto, thick, scale=0.5, every node/.style={scale=0.5, font=\sffamily\normalsize,  rectangle}, small node/.style={rounded rectangle, draw}]
    
   \node (16) [minimum width=5.0cm, minimum height=8.5cm, draw, fill= black!5] at(0,-4.25) {};
   \node (17) [minimum width=5.0cm, minimum height=8.5cm, draw, fill= black!5, right of = 16, node distance = 160] {};
   \node (18) [minimum width=5.0cm, minimum height=8.5cm, draw, fill= black!5, right of = 17, node distance = 160] {};
   \node (1) [small node, minimum width=4.0cm, minimum height=1.2cm, fill= blue!5] {Block \#1};
   \node (2) [small node, minimum width=4.0cm, minimum height=1.2cm, fill= blue!5, node distance = 160, right of = 1] {Block \#2};
   \node (3) [small node, minimum width=4.0cm, minimum height=1.2cm, fill= blue!5, node distance = 160, right of = 2] {Block \#3};
   \node (4) [minimum width=4.5cm, minimum height=4.5cm, draw, fill= green!5, below of = 1, node distance = 90, text depth = 3.5 cm] {Header};
   \node (5) [minimum width=4.5cm, minimum height=4.5cm, draw, fill= green!5, below of = 2, node distance = 90, text depth = 3.5 cm] {Header};
   \node (6) [minimum width=4.5cm, minimum height=4.5cm, draw, fill= green!5, below of = 3, node distance = 90, text depth = 3.5 cm] {Header};
   \node (7) [small node, minimum width=4.0cm, minimum height=1.2cm, fill= white, below of = 1, node distance = 75] {Proof of Work};
   \node (8) [small node, minimum width=4.0cm, minimum height=1.2cm, fill= white, below of = 7, node distance = 45] {Empty Hash};
   \node (9) [small node, minimum width=4.0cm, minimum height=1.2cm, fill= white, right of = 7, node distance = 160] {Proof of Work};
   \node (10) [small node, minimum width=4.0cm, minimum height=1.2cm, fill= white, right of = 8, node distance = 160] {Hash of \#1};
   \node (11) [small node, minimum width=4.0cm, minimum height=1.2cm, fill= white, right of = 9, node distance = 160] {Proof of Work};
   \node (12) [small node, minimum width=4.0cm, minimum height=1.2cm, fill= white, right of = 10, node distance = 160] {Hash of \#2};
   \node (13) [minimum width=4.5cm, minimum height=2.5cm, draw, below of = 8, fill= white, node distance = 80, align=center] {Transaction \#1\\ Transaction \#2\\ Transaction \#3};
   \node (14) [minimum width=4.5cm, minimum height=2.5cm, draw, right of = 13, fill= white, node distance = 160, align=center] {Transaction \#4\\ Transaction \#5\\ Transaction \#6\\ Transaction \#7\\ Transaction \#8};
   \node (15) [minimum width=4.5cm, minimum height=2.5cm, draw, right of = 14, fill= white, node distance = 160, align=center] {Transaction \#9\\ Transaction \#10\\ Transaction \#11};
   \node (19) [right of = 18, node distance = 100] {...};
   
   \path[every node/.style={font=\sffamily\small}] 
   (16) edge node [bend left] {} (10)
   (17) edge node [bend left] {} (12)
   (18) edge node [bend left] {} (19);
          
\end{tikzpicture}
	\caption{The main structure of blockchain. Each block points to the previous one using the hash value. Moreover, blocks hold a varying number of transactions}
	\label{fig:blockchain}
\end{figure*}

\begin{table*}[t]
        \setlength{\tabcolsep}{7pt}
		\renewcommand{\arraystretch}{0.65}
		\centering
		\caption{}
		\label{}
		
		\begin{tabular}{ p{0.1\textwidth} p{0.3\textwidth} p{0.1\textwidth} p{0.3\textwidth} }
		\hline
		 (P1) & Total number of nodes: This represents the number of simulated nodes configured by the user & (P1.1) & Regions of nodes: This represents the geographical location of each node configured by the user.  \\
			\hline
		(P2) & Total number of connections for each node: For each node, this represents the number of possible connections configured by the user. Each node may have a different number of connections & (P3) & Average block propagation delay: This represents the average time delayed in the propagation process of each block configured by the user.\\
			\hline
		(P4) & Average transaction propagation delay:This represents the average time delayed in the propagation process of each transaction  configured by the user & (P5) & Average bandwidth among regions in the network: This represents the average bandwidth assumed for the simulated network  configured by the user.\\
			\hline
		(P6) & Average latency among the simulated regions: This represents the average latency assumed for the simulated network  configured by the user & (P7) & Payload transaction size: This represents the maximum transaction size configured by the user\\
			\hline
		(P8)& Block size: This represents the maximum block size configured by the user & (M1)& Average block size: This represents the average block sizes simulated in the chain simulated in the simulator\\
			\hline
			(M2) & Average block propagation time: This represents the average time taken by the simulator to propagate blocks, simulated in the simulator, in the chain & (M3) & Average transaction propagation time: This represents the average time taken by the simulator to propagate transaction in the simulated chain \\
			\hline
			(M4) & Throughput: This represents the throughput taken by the simulator to the end of the simulations & & \\
			\hline
			(P9) Generate random transactions: This represents the ability to generate automatically generated transactions & (M5) & Chain of block: This represents the resulting chain from the simulator at the end of the simulation\\
			\hline
            (M6) Security: This represents the security assessed by the simulator at the end of the simulation & & \\
			\hline
            (P10) & A Average mining power: This represents the average mining power configured by the user & (P11) & PoW consensus Algorithm: This represents the ability of the simulator to implement PoW consensus algorithm. \\
			\hline
            (P12) Other consensus Algorithm: This represents the ability of the simulator to implement other consensus algorithms than PoW & (P13) Average transaction fee: This represents the average transaction fees configured by the user\\
			\hline
            (P14) Average time for creating a block; aka Block Interval: This represents the average time configured by the user needed to create a block& (M7)& Average block interval: This represents the average time taken, for the blocks to accept transactions, by simulator at the end of the simulation.\\
			\hline
            (M8) Number of generated blocks:  This represents the total number of generated blocks in the simulator  at the end of the simulation & (M9) & Number of mined blocks: This represents the total number of mined blocks by the simulator at the end of the simulation.\\
			\hline
			(M10) & Rate of orphan blocks: This represents the percentage of the orphan blocks by the simulator at the end of the simulation & (M11) & Fork Resolution: This represents whether the simulator maintain the history of blockchain to determine forks occurred as protocol change\\
			\hline
			(P15) & Reward for mine a new block: This represents the amount of reward configured by the user to mine a block & (M12) & Reward for miner: This represents the amount of reward consumed by the simulator at the end of the simulation\\
			\hline
            (M13) & Time of executing a contract: This represents the time taken by the simulator to execute a contract & (M14) & Validation of contract and execution time: This represents how the simulator validates the contract\\
			\hline
			(P16) & Simulation run time: This represents the configured simulation time by the user & (M15)& Resources usage: This represents how the simulator keep track of the resource usage and utilization\\
			\hline
			(M16) & Simulation time: This represents the actual  time taken by the simulator to the end of the simulation & &
			\\
			\hline
		\end{tabular}
	\end{table*}



\subsubsection{Network layer}
\begin{itemize}
    \item (P1) Total number of nodes: This represents the number of simulated nodes configured by the user.
    \item (P1.1) Regions of nodes (unit: geographical): This represents the geographical location of each node configured by the user.
    \item (P2) Total number of connections for each node: For each node, this represents the number of possible connections configured by the user. Each node may have a different number of connections.
    \item (P3) Average block propagation delay (unit: seconds): This represents the average time delayed in the propagation process of each block configured by the user.
    \item (P4) Average transaction propagation delay (unit: seconds):This represents the average time delayed in the propagation process of each transaction  configured by the user.
    \item (P5) Average bandwidth among regions in the network (unit: bits per second): This represents the average bandwidth assumed for the simulated network  configured by the user.
    \item (P6) Average latency among the simulated regions (unit: seconds): This represents the average latency assumed for the simulated network  configured by the user.
    \item (P7) Payload transaction size (unit: Megabyte): This represents the maximum transaction size configured by the user.
    \item (P8) Block size (unit: Megabyte): This represents the maximum block size configured by the user. Note that not all block sizes may reach this limit.
    \item (M1) Average block size: This represents the average block sizes simulated in the chain simulated in the simulator.
    \item (M2) Average block propagation time: This represents the average time taken by the simulator to propagate blocks, simulated in the simulator, in the chain.
    \item (M3) Average transaction propagation time: This represents the average time taken by the simulator to propagate transaction in the simulated chain.
    \item (M4) Throughput (unit: Tx/second): This represents the throughput taken by the simulator to the end of the simulations.
\end{itemize}
\subsubsection{Data layer}
    \begin{itemize}
    \item (P9) Generate random transactions (unit: Integer of Tx per second): This represents the ability to generate automatically generated transactions.
    \item (M5) Chain of block: This represents the resulting chain from the simulator at the end of the simulation.
    \item (M6) Security: This represents the security assessed by the simulator at the end of the simulation.
    \end{itemize}
\subsubsection{Consensus layer}
    \begin{itemize}
    \item (P10) A Average mining power (Hash Rate): This represents the average mining power configured by the user.
    \item (P11) PoW consensus Algorithm: This represents the ability of the simulator to implement PoW consensus algorithm. 
    \item (P12) Other consensus Algorithm: This represents the ability of the simulator to implement other consensus algorithms than PoW.
    \item (P13) Average transaction fee (unit: cryptocurrency): This represents the average transaction fees configured by the user.
    \item (P14) Average time for creating a block; aka Block Interval (unit: seconds): This represents the average time configured by the user needed to create a block.
    \item (M7) Average block interval: This represents the average time taken, for the blocks to accept transactions, by simulator at the end of the simulation.
    \item (M8) Number of generated blocks:  This represents the total number of generated blocks in the simulator  at the end of the simulation.
    \item (M9) Number of mined blocks: This represents the total number of mined blocks by the simulator at the end of the simulation.
    \item (M10) Rate of orphan blocks (unit: percentage): This represents the percentage of the orphan blocks by the simulator at the end of the simulation.
    \item (M11) Fork Resolution: This represents whether the simulator maintain the history of blockchain to determine forks occurred as protocol change.
    \end{itemize}
\subsubsection{Incentive layer}
    \begin{itemize}
    \item (P15) Reward for mine a new block (unit: cryptocurrency): This represents the amount of reward configured by the user to mine a block.
    \item (M12) Reward for miner (unit: cryptocurrency): This represents the amount of reward consumed by the simulator at the end of the simulation.
    \end{itemize}
\subsubsection{Execution layer}
    \begin{itemize}
    \item (M13) Time of executing a contract (unit: seconds): This represents the time taken by the simulator to execute a contract.
    \item (M14) Validation of contract and execution time: This represents how the simulator validates the contract.
    \end{itemize}
\subsubsection{Application layer}
\begin{itemize}
    \item (P16) Simulation run time (unit: seconds): This represents the configured simulation time by the user.
    \item (M15) Resources usage: This represents how the simulator keep track of the resource usage and utilization.
    \item (M16) Simulation time (unit: seconds): This represents the actual  time taken by the simulator to the end of the simulation.
    \end{itemize}
    
    
    \begin{itemize}

    \item Block propagation time: this metric reflects the time taken from sending to receiving a block.
    
    \item Transaction propagation time: this metric reflects the time taken from sending to receiving a transaction.
    
    \item Block size: this metric reflects the average block size generated during the simulation period.
    
    \item Transaction throughput: this metric reflects the rate at which a set of valid committed transactions in a defined time period.
    
    \item Network delay: this metric reflects the total delay occurred in the network.
    
    \item Number of generated block: this metric reflects the total number of the generated blocks during a simulation period.
    
    \item Number of valid block: this metric reflects the total number of valid blocks created during the simulation.
    
    \item Block verification time: this metric reflects the average time taken to verify the generated blocks during the simulation period.
    
    \item Uncle or stale blocks: this metric reflects the number of generated uncle/stale blocks during a simulation period.
    
    \item Fork resolution: this metric reflects whether a fork has ever occurred or not during the simulation.
    
     \item Pending transaction: this metric reflects  the simulators ability to keep track of the transaction number waiting confirmation.
    
    \item Mining difficulty: this metric reflects the amount of difficulty assigned for each transaction.
    
    \item Mining reward: this metric reflects the amount of the used rewards for the mining processes occurred throughout the simulation.
    
    \item Processing speed: this metric reflects the average time taken by the simulator to carry out a specific task during the simulation period.
    
    \item System stability: this metric reflects if the system is stable, in the sense that it can generate a finite set of outputs when given a finite set of inputs.
    
\end{itemize}
